Deterministic Distributed Sparse and Ultra-Sparse Spanners and Connectivity Certificates

This paper presents efficient distributed algorithms for a number of fundamental problems in the area of graph sparsification: We provide the first deterministic distributed algorithm that computes an ultra-sparse spanner in $\textrm{polylog}(n)$ rounds in weighted graphs. Concretely, our algorithm outputs a spanning subgraph with only $n+o(n)$ edges in which the pairwise distances are stretched by a factor of at most $O(\log n \;\cdot\; 2^{O(\log^* n)})$. We provide a $\textrm{polylog}(n)$-round deterministic distributed algorithm that computes a spanner with stretch $(2k-1)$ and $O(nk + n^{1 + 1/k} \log k)$ edges in unweighted graphs and with $O(n^{1 + 1/k} k)$ edges in weighted graphs. We present the first $\textrm{polylog}(n)$-round randomized distributed algorithm that computes a sparse connectivity certificate. For an $n$-node graph $G$, a certificate for connectivity $k$ is a spanning subgraph $H$ that is $k$-edge-connected if and only if $G$ is $k$-edge-connected, and this subgraph $H$ is called sparse if it has $O(nk)$ edges. Our algorithm achieves a sparsity of $(1 + o(1))nk$ edges, which is within a $2(1 + o(1))$ factor of the best possible.

==> todos.tex <==
In addition, there are a few points that are either worth some discussion or are not clear to me.
In Def. 3.2, perhaps we should define the rv E as the indicator rv of the event {E=1} = {\OR_{} X_j = 1}, as opposed to defining it through equality of probabilities.
p.7: X^{i)}_j should be defined as an indicator rv of that the cluster C_j on iteration i is selected. The sentence that appears there suggests that it is the cluster itself.
p.17, par. 2: The sentence "The contribution of each node to both U_i^{uw} and U_i^{w} can be written..." is not clear to me.
p.17, bottom: "These nodes in H aggregates their computed values into the leader of the ND-cluster D."
Does each node sends the actual values for each of the B-S clusters in D, or it does some recomputation of expectations? If it sends the actual values, then how many B-S clusters can actually be contained in a single ND cluster D?
Best,
Michael
